Boosting Randomized Smoothing with Variance Reduced Classifiers

Randomized Smoothing (RS) is a promising method for obtaining robustness certificates by evaluating a base model under noise. In this work, we: (i) theoretically motivate why ensembles are a particularly suitable choice as base models for RS, and (ii) empirically confirm this choice, obtaining state-of-the-art results in multiple settings. The key insight of our work is that the reduced variance of ensembles over the perturbations introduced in RS leads to significantly more consistent classifications for a given input. This, in turn, leads to substantially increased certifiable radii for samples close to the decision boundary. Additionally, we introduce key optimizations which enable an up to 55-fold decrease in sample complexity of RS for predetermined radii, thus drastically reducing its computational overhead. Experimentally, we show that ensembles of only 3 to 10 classifiers consistently improve on their strongest constituting model with respect to their average certified radius (ACR) by 5% to 21% on both CIFAR10 and ImageNet, achieving a new state-of-the-art ACR of 0.86 and 1.11, respectively. We release all code and models required to reproduce our results at https://github.com/eth-sri/smoothing-ensembles.

==> checklist.tex <==
\section*{Checklist}
\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
        \answerYes{We provide a detailed theoretical motivation for our ensembling approach in \cref{sec:theory_var}
        showcasing the claimed results in our evaluation in \cref{sec:eval} and many more in the Appendix. Further, each main contribution in \cref{sec:introduction} explicitly refers to the sections in which it is addressed.}
  \item Did you describe the limitations of your work?
    \answerYes{We discuss the limitations inherent to both Randomized Smoothing in general and our approach in particular in the last paragraph of \cref{sec:eval}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{We provide a discussions of potential societal impacts of our work in \cref{sec:impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We detail the assumptions we make in \cref{sec:theory_var} and provide both empirical as well as theoretical motivations for our choices.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{We include detailed proofs for all derivations in \cref{sec:theory_var} in \cref{sec:math-deriv} and the proof for \cref{thm:adaptive} in \cref{sec:proof_adaptive}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We will make the full code including instructions to reproduce our results publicly available upon publication and add them to the spplemental material for the reviewers. All used data sets are publicly available.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We provide full training details in \cref{sec:experimental-details}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Partially, as due to the high associated cost of training whole ensembles of models multiple times, we only report the variability of our results for one setting in \cref{sec:error-bars}. There, we demonstrate a notable reduction in variance of our ensembles compared to individual models. Upon request we will gladly provide metrics of variability for selected additional experiments.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{As stated in \cref{sec:eval}, we conduct all evaluations for \cifar experiments on single GeForce RTX 2080 Ti and use w for \IN experiments. Further, we provide exact timings for evaluation in \cref{sec:experiment_timings} and training in \cref{sec:details-training}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cite the creators of all frameworks, training methods and datasets we use (see \cref{sec:eval} and \cref{sec:experimental-details}).}
  \item Did you mention the license of the assets?
    \answerYes{For assets explicitly provding a license we mention them in \cref{sec:experimental-details}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We make our code available as supplemental material during the review process and will provide both code as well as pretrained models via URL upon publication. No other new assets are being introduced.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Only public datasets were used.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Only standard, public datasets were used.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> evaluation_theory.tex <==
\subsubsection{Empirical Analysis of Theoretical Results} \label{sec:exp_theory}

We validate and instantiate our theoretical analysis for the example of an ensemble of $k=50$ \RNS trained as per \citet{CohenRK19}. We obtain $c$ and $\Sigma_{c}$ as the mean and covariance of the output on a randomly chosen sample. Subtracting the clean output of every classifier from that for  samples perturbed with $\sigma = 0.25$ and enforcing zero mean, we obtain the covariance matrix $\Sigma_{p}$. We determine both $\zeta_c$ and $\zeta_p$ by computing all pairwise covariances between all logits of two classifiers and computing the median ratio between the thus obtained inter-classifier covariance with the intra-classifier covariance. 
We observe $\zeta_c \approx 0$ and $\zeta_p \approx 0.82$ ($\mu_{\zeta_p} = 0.820 $ and $\sigma^2_{\zeta_p} = 0.0023$).



\begin{figure}[t]
	\centering
	\makebox[\textwidth][c]{
	\begin{subfigure}[t]{0.33\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/runner_up_margin-eps-converted-to.pdf}
		\label{fig:class_margin_distr}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.274\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figures/succes_prob-eps-converted-to.pdf}
		\label{fig:p_success}
	\end{subfigure}
		\hfill
	\begin{subfigure}[t]{0.322\textwidth}
	\centering
	\includegraphics[width=1.1\linewidth]{./figures/cert_rad_distr-eps-converted-to.pdf}
	\label{fig:cert_rad_distr}
	\end{subfigure}
}
	\vspace{-5mm}
	\caption{Comparison of the (a) modeled distribution over the classification margin to the runner up class, (b) the resulting success probability of predicting the majority class for a given perturbation, and (c) the corresponding distribution over certified radii for ensembles of different size.}
	\label{fig:exp_theory}
\end{figure}


Instantiating our Gaussian model from \cref{sec:theory_var_gauss} with these parameters, we observe that while the mean classification margin to the runner up class (see \cref{fig:exp_theory} (a)) remains the same, its variance is decreased significantly. As the probability of predicting the majority class is effectively equal to the area under the corresponding curve on the right hand side of the decision threshold $\bar{z} = 0$, this translates to a marked increase in the probability of the ensemble predicting the majority class for any given perturbation (see \cref{fig:exp_theory} (b)). This increase in success probability in turn translates into a much larger expected certified radius (see \cref{fig:exp_theory} (c)) for a given number of sampled perturbations (here $n = 10^3$). For this example, the expected certified radius (over randomness in the sampling process) increases almost 3-fold from $0.086$ for a single model to $0.253$ for an ensemble of $k=50$ models. In contrast, sampling more for the same success probability will in the limit only recover the true success probability for an ensemble of a given size. In this scenario for example, increasing the number of samples drawn for a single model  $50$-fold (matching the number of model evaluations of the ensemble of 50 models), only increases the expected certified radius to $0.110$.

\begin{wrapfigure}{r}{0.35\textwidth}
	\centering
	\vspace{-5mm}
	\includegraphics[width=1.0\linewidth]{./figures/ecr_samples-eps-converted-to.pdf}
	\caption{Expected certified radius over the number $n$ of samples for the true success probabilities $p_A$.}
	\label{fig:cert_rad_p}
\end{wrapfigure}
This observation however, only holds for samples close to the decision boundary. When the whole probability mass of the classification margin distribution is far to the right of the decision threshold, the success probability $p_A$ will already be close to $1$ for an individual classifier, and the confidence lower bound to the success probability  $\underline{p_A}$ is dominated by the number of samples, making an individual classifier is more efficient. This effect can be seen in \cref{fig:cert_rad_p} where the expected certified radius is illustrated as a function of the number of samples.

==> table_cifar10_10_ensemble_adaptive_sampling_025_consistency.tex <==
\begin{table}[t]
	\centering
	\small
	\centering
	\caption{Effect of adaptive sampling with $\{n_j\} = \{1'000, 10'000, 125'000\}$ for ensembles of $10$ \consistency trained \RNB on \IN at $\sigma_{\epsilon} = 0.25$. ASA$_j$ and ASC$_j$ are the percentages of samples abstained from and certified in phase $j$, respectively}
	\label{tab:adaptive_ensemble_consistency}
	\scalebox{0.9}{
	\begin{tabular}{cccccccccc}
		\toprule
        Radius & acc$_{\text{cert}}$ [\%] & ASA$_1$ & ASC$_1$ & ASA$_2$ & ASC$_2$ & ASA$_3$ & ASC$_3$ & SampleRF & TimeRF\\
        \midrule
        0.25 & 70.4 & 15.2 & 80.6 & 0.6 & 3.0 & 0.6 & 0.0 & \textbf{46.17} & \textbf{43.29}\\
        0.50 & 60.4 & 26.0 & 64.8 & 4.2 & 2.0 & 2.0 & 1.0 & 18.61 & 17.27\\
        0.75 & 52.0 & 36.4 & 0.0 & 3.6 & 51.4 & 3.4 & 5.2 & 5.99 & 5.49\\
		\bottomrule
	\end{tabular}
}
\end{table}

==> table_cifar10_adaptive_sampling_ablation_075.tex <==
\begin{table}[t]
	\centering
	\small
	\centering
	\caption{Adaptive sampling ablation study for radius $0.75$ with one ResNet110 each. First half is trained with Cohen, second half is trained with consistency.}
	\resizebox{0.97\columnwidth}{!}{
	\begin{tabular}{cccccccccccccc}
		\toprule
        ID & CertAcc [\%] & P1A [\%] & P1C [\%] & P1CC [\%] & P2A [\%] & P2C [\%] & P2CC [\%] & P3A [\%] & P3C [\%] & P3CC [\%] & SampleGain & Time [h] & TimeGain\\
        \midrule
        0 & 30.4 & 59.8 & 0.0 & 0.0 & 9.6 & 30.6 & 30.4 & 0.0 & 0.0 & 0.0 & 2.13 & 1.94 & 2.18\\
        1 & 30.4 & 65.0 & 24.6 & 24.4 & 4.4 & 6.0 & 6.0 & 0.0 & 0.0 & 0.0 & 4.76 & 0.90 & 4.70\\
        2 & 30.6 & 61.2 & 0.0 & 0.0 & 3.8 & 24.8 & 24.6 & 4.2 & 6.0 & 6.0 & 6.13 & 0.73 & 5.82\\
        3 & 30.6 & 61.2 & 0.0 & 0.0 & 4.2 & 27.6 & 27.4 & 3.8 & 3.2 & 3.2 & 6.74 & 0.68 & 6.19\\
        \midrule
        0 & 46.4 & 41.2 & 0.0 & 0.0 & 9.6 & 49.2 & 46.4 & 0.0 & 0.0 & 0.0 & 1.47 & 2.87 & 1.47\\
        1 & 46.4 & 46.6 & 43.6 & 41.8 & 4.2 & 5.6 & 4.6 & 0.0 & 0.0 & 0.0 & 4.91 & 0.90 & 4.72\\
        2 & 46.2 & 40.6 & 0.0 & 0.0 & 5.8 & 44.0 & 42.0 & 4.6 & 5.0 & 4.2 & 5.72 & 0.80 & 5.27\\
        3 & 46.6 & 43.2 & 0.0 & 0.0 & 4.4 & 45.0 & 42.8 & 3.0 & 4.4 & 3.8 & 5.68 & 0.83 & 5.08\\
		\bottomrule
	\end{tabular}
}
\end{table}

==> table_cifar10_adaptive_sampling_ablation_5_phases.tex <==
\begin{table}[t]
	\centering
	\small
	\centering
	\caption{Adaptive sampling for $5$ phases. ID $0$ represents $\{1000, 4000, 16000, 64000, 13000\}$, $1$ represents $\{100, 1000, 5000, 25000, 130000\}$. \todo{Add this to the appendix}}
	\resizebox{0.97\columnwidth}{!}{
	\begin{tabular}{ccccccccccccccccc}
		\toprule
        Training & Radius & ID & CertAcc [\%] & P1A [\%] & P1C [\%] & P2A [\%] & P2C [\%] & P3A [\%] & P3C [\%] &  P4A [\%] & P4C [\%] &  P5A [\%] & P5C [\%] & SampleGain & Time [h] & TimeGain\\
        \midrule
        Gaussian & 0.25 & 0 & 60.2 & 29.2 & 61.2 & 2.8 & 1.6 & 1.6 & 1.2 & 0.8 & 1.0 & 0.2 & 0.4 & 28.12 & 0.20 & 20.65\\
        Gaussian & 0.25 & 1 & 60.0 & 19.8 & 53.2 & 10.6 & 7.8 & 2.0 & 2.0 & 1.2 & 0.8 & 1.4 & 1.2 & 22.56 & 0.24 & 17.25\\
        \midrule
        Consistency & 0.25 & 0 & 66.0 & 20.2 & 74.8 & 1.4 & 0.6 & 0.6 & 0.8 & 0.8 & 0.2 & 0.4 & 0.2 & 36.09 & 0.16 & 26.89\\
        Consistency & 0.25 & 1 & 66.0 & 12.8 & 68.4 & 8.0 & 6.2 & 1.2 & 1.2 & 0.6 & 0.4 & 0.8 & 0.4 & 44.43 & 0.12 & 33.73\\
        \midrule
        Gaussian & 0.75 & 0 & 30.6 & 59.6 & 0.0 & 4.0 & 0.0 & 2.8 & 26.8 & 1.2 & 3.4 & 1.6 & 0.6 & 8.78 & 0.69 & 6.15\\
        Gaussian & 0.75 & 1 & 30.6 & 48.2 & 0.0 & 11.4 & 0.0 & 3.8 & 0.0 & 3.2 & 29.0 & 2.6 & 1.8 & 7.04 & 0.77 & 5.45\\
        \midrule
        Consistency & 0.75 & 0 & 46.6 & 40.6 & 0.0 & 4.0 & 0.0 & 3.0 & 45.0 & 1.2 & 4.2 & 1.8 & 0.2 & 6.95 & 0.85 & 4.97\\
        Consistency & 0.75 & 1 & 46.2 & 32.6 & 0.0 & 8.6 & 0.0 & 4.2 & 0.0 & 2.4 & 46.4 & 3.2 & 2.6 & 4.96 & 1.09 & 3.88\\
		\bottomrule
	\end{tabular}
}
\end{table}

==> table_cifar10_ensemble_size_ablation_short.tex <==
\begin{table}[t]
	\centering
	\small
	\centering
	\caption{Ensemble Size Study with \RNS. First half uses $\sigma=0.25$ for training and evaluation, the other $\sigma=1.00$.}
	\resizebox{0.97\columnwidth}{!}{
	\begin{tabular}{lllccccccccccccc}
		\toprule
        Training& $\sigma$ & $k$ & ACR& $r = 0.0$& $r = 0.25$& $r = 0.5$& $r = 0.75$& $r = 1.0$& $r = 1.25$& $r = 1.5$& $r = 1.75$& $r = 2.0$& $r = 2.25$& $r = 2.5$\\
        \midrule
        \multirow{10}{*}{Cohen}&\multirow{5}{*}{0.25}& 1& 0.434 & 77.4 & 63.4 & 43.6 & 26.6 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
		& & 5 & 0.500 & 80.2 & 65.4 & 50.4 & 36.8 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
		& & 10& 0.510 & \textbf{80.4} & 67.4 & 51.8 & 37.4 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
		& & 50 & \textbf{0.517} & \textbf{80.4} & \textbf{68.6} & \textbf{52.8} & \textbf{38.8} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
		\cmidrule(lr){2-2}
		&\multirow{5}{*}{1.0}& 1 & 0.538 & 48.0 & 41.2 & 35.0 & 27.8 & 21.6 & 17.8 & 14.8 & 12.0 & 9.0 & 5.6 & 3.4\\
		& & 5  & 0.590 & 49.2 & 42.8 & \textbf{37.8} & \textbf{30.4} & \textbf{24.0} & \textbf{19.4} & \textbf{16.2} & \textbf{13.8} & \textbf{11.2} & 8.2 & \textbf{5.0}\\
		& & 10 & 0.592 & 48.8 & 42.8 & 37.0 & \textbf{30.4} & 23.6 & 19.0 & 16.2 & 13.6 & 11.0 & \textbf{9.2} & \textbf{5.0}\\
		& & 50& \textbf{0.597} & \textbf{49.6} & \textbf{43.0} & 37.4 & \textbf{30.4} & 23.6 & 18.6 & 15.8 & 13.6 & \textbf{11.2} & 9.0 & \textbf{5.0}\\
  		\cmidrule(lr){1-2}
        \multirow{10}{*}{Consistency}& \multirow{5}{*}{0.25} & 1 & 0.528 & 71.8 & 64.2 & 55.6 & 45.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
        & & 5 & 0.547 & \textbf{73.0} & \textbf{65.4} & \textbf{57.6} & 47.6 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
        & & 10& 0.547 & 72.2 & 65.0 & 57.4 & 48.8 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
        & & 50& \textbf{0.551} & \textbf{73.0} & 64.8 & 57.0 & \textbf{50.2} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
		\cmidrule(lr){2-2}
        &\multirow{5}{*}{1.0} &1 & 0.757 & 43.6 & 39.8 & 34.8 & 30.8 & 27.6 & 24.6 & \textbf{22.6} & 19.4 & 17.4 & 15.4 & 13.8\\
        & & 5 & 0.779 & 43.4 & 40.0 & 35.6 & 32.2 & 28.0 & 24.8 & 22.2 & \textbf{20.4} & 17.4 & 15.8 & 13.8\\
        & & 10& 0.784 & 44.4 & \textbf{40.6} & \textbf{36.4} & 32.2 & \textbf{29.2} & 24.2 & 22.2 & \textbf{20.4} & 17.6 & \textbf{16.0} & 14.2\\
        & & 50& \textbf{0.788} & \textbf{45.2} & \textbf{40.6} & \textbf{36.4} & \textbf{32.4} & 28.2 & 24.6 & 22.0 & 20.2 & \textbf{17.8} & \textbf{16.0} & \textbf{14.6}\\
		\bottomrule
	\end{tabular}
}
\end{table}

==> table_cifar10_main_short.tex <==
\begin{table}[t]
	\centering
	\small
	\centering
	\caption{\cifar average certified radius (ACR) and certified accuracy at different radii for ensembles of $k$ models ($k=1$ are individual models) with \RNB architecture and $\sigma_{\epsilon} = 0.5$. Larger is better.}
	\label{tab:cifar10_main_short}
	\scalebox{0.83}{
	\begin{threeparttable}
		\begin{tabular}{ccccccccccc}
			\toprule
			\multirow{2.6}{*}{Training} &\multirow{2.6}{*}{$k$} & \multirow{2.6}{*}{ACR} & \multicolumn{8}{c}{Radius r}\\
			\cmidrule(lr){4-11}
			& & & 0.0 & 0.25 & 0.50 & 0.75 & 1.00 & 1.25 & 1.50 & 1.75 \\
			

			\midrule
			\multirow{2}{*}{\cohen} & 1 & 0.535 & 65.8 & 54.2 & 42.2 & 32.4 & 22.0 & 14.8 & 10.8 & 6.6 \\
			& 10 & 0.648 & \textbf{69.0} & \textbf{60.4} & \textbf{49.8} & 40.0 & 29.8 & 19.8 & 15.0 & 9.6 \\
			\cmidrule(lr){1-1}
			\multirow{2}{*}{\consistency} & 1 & 0.708 & 63.2 & 54.8 & 48.8 & 42.0 & 36.0 & 29.8 & 22.4 & 16.4 \\
			& 10 & \textbf{0.756} & 65.0 & 59.0 & 49.4 & \textbf{44.8} & 38.6 & 32.0 & 26.2 & 19.8 \\
			\cmidrule(lr){1-1}
			\multirow{2}{*}{\smoothadv} & 1 & 0.707 & 52.6 & 47.6 & 46.0 & 41.2 & 37.2 & 31.8 & 28.0 & 23.4 \\
			& 10 & 0.730 & 52.4 & 48.6 & 45.8 & 42.6 & \textbf{38.8} & \textbf{34.4} & \textbf{30.4} & \textbf{25.0} \\
			\cmidrule(lr){1-1}
			\macer & 1 & 0.668 & 62.4 & 54.4 & 48.2 & 40.2 & 33.2 & 26.8 & 19.8 & 13.0 \\
			
	
			\bottomrule
		\end{tabular}
\end{threeparttable}
}
\vspace{-5mm}
\end{table}


==> table_ensemble_size.tex <==
\begin{wraptable}[7]{r}{0.34\textwidth}
	\vspace{-0.5mm}	
	\small
	\centering
	\caption{\cohen trained ensembles of different size on \cifar at $\sigma_{\epsilon}=0.25$}
	\vspace{-2mm}
	\scalebox{0.82}{
	\begin{tabular}{ccccccc}
		\toprule
		\multirow{2.6}{*}{Architecture} & \multirow{2.6}{*}{$k$} & \multirow{2.6}{*}{ACR} & \multicolumn{4}{c}{Radius r}\\
         \cmidrule(lr){4-7}
         & & & 0.0 & 0.25 & 0.50 & 0.75 \\
        \midrule
		\multirow{2}{*}{\RNB} & 1 & 0.450 & 77.6 & 60.0 & 45.6 & 30.6 \\
							  & 10 & 0.541 & \textbf{83.4} & \textbf{70.6} & 55.4 & 42.0 \\
		\cmidrule(lr){2-2}
		\multirow{3}{*}{\RNS} & 1 & 0.434 & 77.4 & 63.4 & 43.6 & 26.6 \\
							  & 5 & 0.500 & 80.2 & 65.4 & 50.4 & 36.8 \\
							  & 50 & 0.517 & 80.4 & 68.6 & 52.8 & 38.8\\
  
		\bottomrule
	\end{tabular}
}
\end{wraptable}

==> table_imagenet_adaptive_consistency3_short.tex <==
\begin{table}[t]
	\centering
	\small
	\centering
	\caption{Adaptive sampling with $\{n_j\} = \{1'500, 15'000, 125'000\}$ on ImageNet with an ensemble of $3$ \consistency trained \RNM. Sample and time gain are the reduction factor in comparison to standard sampling with $n=100'000$ on the same ensemble (larger is better). $ASR_j$ is the ratio of samples returned in phase $j$.}%
	\label{tab:IN_adaptive_short}
	\resizebox{0.83\columnwidth}{!}{
	\begin{tabular}{ccccccc}
		\toprule
		Radius & $\text{acc}_{\text{cert}}$ [\%] & $ASR_1$ [\%] & $ASR_2$ [\%] & $ASR_3$ [\%] & Sample Gain & Time Gain \\
        \midrule
        0.50 & 40.2 & 93.8 & 4.4 & 1.8 & 22.66 & 20.7\\
        1.00 & 37.2 & 95.0 & 4.0 & 1.0 & \textbf{29.66} & \textbf{27.5}\\
        2.00 & 28.6 & 89.8 & 8.6 & 1.6 & 21.13 & 19.3\\
        3.00 & 19.8 & 70.0 & 25.6 & 4.4 & 9.54 & 8.6\\
		\bottomrule
	\end{tabular}
	}
\vspace{-4mm}
\end{table}

==> table_imagenet_main_short.tex <==
\begin{table}[t]
			\centering
			\small
			\caption{\IN average certified radius (ACR) and certified accuracy at different radii for ensembles of $k$ \RNM ($k=1$ are individual models) at various $\sigma_{\epsilon}$. Larger is better.} 
			\label{tab:IN_main_short}
			\scalebox{0.77}{
			\begin{threeparttable}
				\begin{tabular}{cccccccccccc}
					\toprule
					\multirow{2.6}{*}{$\sigma_{\epsilon}$} & \multirow{2.6}{*}{Training} & \multirow{2.6}{*}{$k$} & \multirow{2.6}{*}{ACR} & \multicolumn{8}{c}{Radius r}\\
					\cmidrule(lr){5-12}
					& & & & 0.0 & 0.50 & 1.00 & 1.50 & 2.00 & 2.50 & 3.00 & 3.50 \\
			
					
					\midrule
					\multirow{8.5}{*}{0.25} & \cohen & 1 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\
					\cmidrule(lr){2-3}
					& \smoothadv & 1 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\
					\cmidrule(lr){2-3}
					& \macer & 1 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\
					\cmidrule(lr){2-3}
					& \multirow{2}{*}{\consistency} & 1 & 0.516 & 64.8 & 54.2 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
					\cmidrule(lr){3-3}
					& & 3 & \textbf{0.545} & \textbf{65.6} & \textbf{57.0} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
					
			
					\midrule
					\multirow{8.5}{*}{0.5} & \cohen & 1 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\
					\cmidrule(lr){2-3}
					& \smoothadv & 1 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\
					\cmidrule(lr){2-3}
					& \macer & 1 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\
					\cmidrule(lr){2-3}
					& \multirow{2}{*}{\consistency} & 1 & 0.806 & 55.4 & 48.8 & 42.2 & 35.0 & 0.0 & 0.0 & 0.0 & 0.0\\
					\cmidrule(lr){3-3}
					& & 3 & \textbf{0.868} & 57.0 & \textbf{52.0} & \textbf{44.6} & \textbf{38.4} & 0.0 & 0.0 & 0.0 & 0.0\\
			
					\midrule
					\multirow{14.5}{*}{1.0} & \multirow{2}{*}{\cohen} & 1 & 0.856 & 42.4 & 37.2 & 31.4 & 25.8 & 19.6 & 15.4 & 12.0 & 8.4\\
					\cmidrule(lr){3-3}
					& & 3 & 0.968 & 43.8 & 38.4 & 34.4 & 29.8 & 23.2 & 18.2 & 15.4 & 11.4\\
					\cmidrule(lr){2-3}
					& \multirow{2.0}{*}{\smoothadv} & 1 & 1.011 & 40.6 & 38.6 & 33.8 & 29.8 & 25.6 & 20.6 & 18.0 & 14.4 \\
					\cmidrule(lr){3-3}
					&   & 3 & 1.065 & 38.6 & 36.0 & 34.0 & 30.0 & 27.6 & \textbf{24.6} & \textbf{21.2} & \textbf{18.8} \\
					\cmidrule(lr){2-3}
					& \macer & 1 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 & -1.0 \\
					\cmidrule(lr){2-3}
					& \multirow{2.0}{*}{\consistency} & 1 & 1.022 & 43.2 & 39.8 & 35.0 & 29.4 & 24.4 & 22.2 & 16.6 & 13.4 \\
					\cmidrule(lr){3-3}
					& &  3 & \textbf{1.108} & 44.6 & 40.2 & \textbf{37.2} & \textbf{34.0} & \textbf{28.6} & 23.2 & 20.2 & 16.4 \\
			
					\bottomrule
				\end{tabular}
			\begin{tablenotes}
				\item[$\dagger$]{As reported by \citet{zhai2020macer}.}
		\end{tablenotes}
		\end{threeparttable}
		}
\vspace{-4mm}
\end{table}


==> table_natural_accuracy.tex <==
\begin{table}[t]
	\centering
	\small
	\centering
	\caption{Absolute and relative improvements of $10$ \RNB compared to $1$ \RNB for \cohen and \consistency trained models on \cifar with $\sigma_{\epsilon}=0.50$. We consider various certified radii $r$, as well as the natural accuracy (NAC) which we obtain by testing on clean samples.}
	\label{tab:natural_accuracy}
	\resizebox{0.935\columnwidth}{!}{
	\begin{threeparttable}
	\begin{tabular}{ccccccccccc}
		\toprule
		\multirow{2.6}{*}{Improvement [\%]} & \multirow{2.6}{*}{Training} & \multirow{2.6}{*}{NAC} & \multicolumn{8}{c}{Radius r}\\
		\cmidrule(lr){4-11}
		& & & 0.00 & 0.25 & 0.50 & 0.75 & 1.00 & 1.25 & 1.50 & 1.75\\
        \midrule
        \multirow{2}{*}{Absolute} & \cohen & 2.2 & 3.2 & 6.2 & 7.6 & 7.6 & 7.8 & 5.0 & 4.2 & 3.0\\
        & \consistency & 2.0 & 1.8 & 4.2 & 0.6 & 2.8 & 2.6 & 2.2 & 3.8 & 3.4\\
        \midrule
        \multirow{2}{*}{Relative} & \cohen & 3.08 & 4.86 & 11.44 & 18.01 & 23.46 & 35.43 & 33.78 & 38.89 & 45.45\\
        & \consistency & 3.08 & 2.85 & 7.66 & 1.23 & 6.67 & 7.22 & 7.38 & 16.96 & 20.7\\
		\bottomrule
	\end{tabular}
\end{threeparttable}
}
\end{table}



